Beyond Gauss: Image-Set Matching on the Riemannian Manifold of PDFs

State-of-the-art image-set matching techniques typically implicitly model each image-set with a Gaussian distribution. Here, we propose to go beyond these representations and model image-sets as probability distribution functions (PDFs) using kernel density estimators. To compare and match image-sets, we exploit Csiszar f-divergences, which bear strong connections to the geodesic distance defined on the space of PDFs, i.e., the statistical manifold. Furthermore, we introduce valid positive definite kernels on the statistical manifolds, which let us make use of more powerful classification schemes to match image-sets. Finally, we introduce a supervised dimensionality reduction technique that learns a latent space where f-divergences reflect the class labels of the data. Our experiments on diverse problems, such as video-based face recognition and dynamic texture classification, evidence the benefits of our approach over the state-of-the-art image-set matching methods.

==> sec_intro.tex <==
\section{Introduction}
\label{sec:intro}

This paper tackles the problem of image-set matching by comparing probability distribution functions (PDFs) using 
Csisz\'{a}r $f$-divergences~\cite{Csiszar_1963,Ali_1966}.
Image-set matching, \ie matching unordered sets of images, exploits the richer information contained in multiple images to perform recognition.
With the growth of camera networks, video data, hyper-spectral imaging technologies, \etc.,
image-sets are becoming ubiquitous in our everyday lives.
% as evidenced by the surge of publications in this domain\footnote{To the best of our knowledge, at least 6 papers have tackled this problem among the accpeted papers to CVPR-2015.}.

State-of-the-art image-set matching methods~\cite{Hamm_ICML_2008,Wang_CVPR_2012,Harandi_ICCV_2013,Huang_PR_2015} typically model image-sets using geometrical structures, \eg, Riemannian manifolds.
The two most popular such structures are Grassmann manifolds~\cite{Absil_2008} and the manifold of Symmetric Positive Definite (SPD) matrices~\cite{Pennec_IJCV_2006}. 
From a different perspective, these representations can be related to modeling an image-set with a single multivariate Gaussian distribution. Indeed, in the case of the SPD manifold~\cite{Wang_CVPR_2012}, an image-set is represented as the covariance matrix of the features extracted in each image of the set, which therefore essentially encodes a zero-mean Gaussian distribution of the image features. For Grassmann manifolds, where an image-set is represented by a subspace of its image features,~\cite{Hamm_NIPS_2009} related several distances between subspaces to distances between multivariate Gaussian distributions. While both manifolds have been shown to provide representations that are robust to varying imaging conditions, intuitively, modeling an image-set with a single Gaussian distribution seems restrictive. 

In this paper, we therefore propose to make use of better probabilistic models to represent an image-set and study different ways to compare such models for the task of image-set matching.
To this end, we model the PDF of an image-set using a non-parametric, data-driven kernel density estimator. Since PDFs form a Riemannian manifold, \ie, the {\it statistical manifold}, the geodesic distance on the manifold comes as a natural choice to measure the similarity between two image-sets. Unfortunately, the geodesic distance is impractical to compute for general distributions. Therefore, we propose to exploit Csisz\'{a}r $f$-divergences~\cite{Csiszar_1963}, which bear strong connections to the geodesic distance. In particular, we study two specific $f$-divergences and discuss how robust empirical estimates of these divergences can be obtained.

From a recognition perspective, $f$-divergences can be directly employed in a nearest neighbor classifier to match image-sets. 
However, for complex recognition tasks, a nearest neighbor classifier may have limited power.
%While $f$-divergences can be directly employed to match image-sets, 
%such a nearest-neighbor classifier may have limited power in practice. 
To address this issue, we therefore study the positive definiteness of kernels induced by these $f$-divergences. 

\textcolor{red}{
Jaakkola and Haussler introduced a general form of positive definite kernels on statistical manifolds~\cite{Jaakkola_NIPS_1999}. 
The kernels in~\cite{Jaakkola_NIPS_1999} are characterized by the Fisher information matrix, hence the kernels are defined for statistical
models that can be described by a finite set of parameters. In contrast, the kernel developed in this work relaxes that assumption 
and is positive definite in the most general form.   
}

Finally, to account for the fact that the image features may not be the best representation to compare the data, we introduce a dimensionality reduction approach that exploits the 
\textcolor{red}{$f$-divergences} between image-sets. More specifically, we search for a low-dimensional space where the $f$-divergence between image-sets from different classes is maximized, while the $f$-divergence between image-sets of the same class is minimized. We then show that, thanks to a property of the $f$-divergences, dimensionality reduction can be cast as a minimization problem on a Grassmann manifold.

Our contributions can be summarized as: 
\textbf{1.} We introduce a new representation of image-sets as %fine-grained, 
non-parametric PDFs.
\textbf{2.} We propose to make use of $f$-divergences to perform image-set matching.
\textbf{3.} We introduce a family of positive definite kernels on the space of PDFs.
%and consequently use them to transform problems modeled by PDFs into familiar problems in Reproducing Kernel Hilbert Spaces (RKHS).
\textbf{4.} We derive a supervised dimensionality reduction technique that maximizes a notion of discriminative power between PDFs. 

We evaluate the different algorithms derived from our analysis on several image-set matching tasks, including 
face recognition, dynamic texture categorization and scene classification. Our experiments evidence the benefits of our approach over state-of-the-art image-set matching methods. In particular, we outperform the state-of-the-art on the Youtube celebrity~\cite{YT_Celebrity},
DynTex++~\cite{DynTex_Dataset},
UCSD traffic~\cite{Chan_CVPR2005} and Maryland scene recognition~\cite{Shroff_CVPR_2010} datasets.%, and match its performance on other data.



\subsection{Related Work}

As mentioned above, our work is motivated by methods that rely on geometrical structures, such as SPD and Grassmann manifolds, to represent image-sets, since they can be related to modeling image sets with Gaussian distributions. We therefore focus our discussion on those methods.

%\cite{Mian_TIP_2013} {\bf WHAT DO THEY DO? THIS WAS LISTED AS A GEOMETRICAL METHOD AND SHOULD THEREFORE PROBABLY BE DISCUSSED IN ONE OF THE FOLLOWING TWO PARAGRAPHS. IT IS STILL UNDER METRIC LEARNING IN THE LAST PARAGRAPH.}

In the context of SPD manifolds, Wang \etal proposed to model each image-set by a covariance matrix~\cite{Wang_CVPR_2012}. This allowed the authors to exploit the Riemannian geometry of SPD matrices to analyze image-sets. More specifically,~\cite{Wang_CVPR_2012} made use of a kernel function on the SPD manifold to perform kernel partial least squares regression or kernel discriminant analysis to recognize human faces in videos. Following this,~\cite{Huang_PR_2015} proposed to learn a combination of various kernels, including kernels on SPD manifolds, to boost the recognition accuracy.
%~\cite{Rosipal_JMLR_2002} 

The use of subspaces to match image-sets can be traced back to~\cite{Yamaguchi_FGR_1998}. The main idea is to fit a subspace to the samples of an image-set and utilize the distance between multiple subspaces for classification. With the advance of methods that exploit the geometry of Grassmann manifolds, more sophisticated classifiers have been employed. For instance, Hamm and Lee~\cite{Hamm_ICML_2008} proposed to embed the Grassmannian into a Reproducing Kernel Hilbert Space (RKHS) and perform discriminant analysis in the resulting space. In~\cite{Harandi_ICCV_2013}, notions of sparse coding on the Grassmann manifold were utilized to perform image-set classification. 

Since a covariance matrix inherently encodes a single Gaussian, and since several metrics between subspaces have been shown to be equivalent to distances between Gaussian distributions~\cite{Hamm_NIPS_2009}, 
both covariance-based and subspace-based representations can be related to modeling an image-set with a single multivariate Gaussian distribution. Note that Arandjelovic \etal~\cite{Arandjelovic_CVPR_2005} proposed to go beyond a single Gaussian by exploiting a Gaussian mixture model (GMM) in a low-dimensional space to represent an image-set. The similarity between to GMMs was then computed by a Monte-Carlo method. Here, in contrast, we make use of non-parametric density estimation along robust empirical estimate of the distance between two PDFs. Furthermore, we define valid kernels on the statistical manifold and learn a low-dimensional representation that implicitly accounts for the $f$-divergence between the PDFs.

Of course, many other image-set matching techniques have been devised in the past, including deep networks~\cite{Hayat_PAMI_2015,Lu_CVPR_2015}, sparse coding and 
dictionary learning~\cite{Lu_ECCV_2014} and metric learning~\cite{Vemulapalli_CVPR_2013,Mian_TIP_2013}.
%, and convex and affine hull models~\cite{Cevikalp_CVPR_2010}. 
While discussing these approaches in details goes beyond the scope of this paper, our experiments, which compare our results with the state-of-the-art in each dataset, demonstrate the benefits of our approach over these baselines.
 
%Both manifolds have shown to provide more robust models for encoding image-sets. For example, in the case of SPD manifolds,
%one could use an affine invariant metric for comparing image-sets. Needless to say that affine invariance 
%is attractive for vision applications. As another example, illumination cone is a low-dimensional subspace~\cite{Belhumeur_IJCV_1998}
%and hence encoding image-sets by subspaces may result in robustness against illumination variation.


